ST-Gait++: Leveraging spatio-temporal convolutions for gait-based emotion recognition on videos

Emotion recognition is relevant for human behaviour understanding, where facial expression and speech recognition have been widely explored by the computer vision community. Literature in the field of behavioural psychology indicates that gait, described as the way a person walks, is an additional indicator of emotions. In this work, we propose a deep framework for emotion recognition through the analysis of gait. More specifically, our model is composed of a sequence of spatial-temporal Graph Convolutional Networks that produce a robust skeleton-based representation for the task of emotion classification. We evaluate our proposed framework on the E-Gait dataset, composed of a total of 2177 samples. The results obtained represent an improvement of approximately 5% in accuracy compared to the state of the art. In addition, during training we observed a faster convergence of our model compared to the state-of-the-art methodologies.

==> tables/table-result-search-bayes.tex <==
\begin{table}[H]
\caption{Results for the Bayesian Search.}
\label{tbl:resultsSearchSpaceBayes}
\centering
\resizebox{\columnwidth}{!}{\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}c }
\hline
\textbf{Parameters} & \textbf{Chosen Value} \\ \hline
Basic Learning Rate & 0.01                  \\
GCN Initializer     & Offset                \\
Optimizer           & RMSProp               \\
Weight Decay        & $3 \times 10^{-4}$    \\ \hline
\end{tabular}}
\end{table}

==> tables/table-results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{table}[H]
\caption{Accuracy values and convergence epochs for STEP and ST-Gait++.}
\label{tbl:result-training}
\centering
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{lccc}
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Accuracy (\%)}}                                                                       \\ \cline{2-4} 
                                & \multicolumn{1}{l}{\textbf{Test}} & \multicolumn{1}{l}{\textbf{Validation}} & \multicolumn{1}{l}{\textbf{Train}} \\ \hline
STEP                            & 83.3                             & 78.9                                   & 82.9                              \\
\textbf{ST-Gait++}              & \textbf{87.5}                     & \textbf{78.7}                           & \textbf{91.8}                     \\ \hline
\end{tabular}
\end{table}

% \begin{tabular}{|c|ccc|c|}
% \hline
% \rowcolor[HTML]{9B9B9B} 
% \cellcolor[HTML]{C0C0C0}                                 & \multicolumn{3}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{Accuracy}}                                                                                    & \cellcolor[HTML]{C0C0C0}                                 \\ \cline{2-4}
% \rowcolor[HTML]{C0C0C0} 
% \multirow{-2}{*}{\cellcolor[HTML]{C0C0C0}\textbf{Model}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Test}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Validation}} & \textbf{Training} & \multirow{-2}{*}{\cellcolor[HTML]{C0C0C0}\textbf{Epoch}} \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% STEP                                                     & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}83,33\%}       & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}78,94\%}             & 82,96\%           & 462                                                      \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% ST-Gait++                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}87,5\%}        & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}78,70\%}             & 91,84\%           & 127                                                      \\ \hline
% \end{tabular}
% \end{table}

==> tables/table-skeleton-coord.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[H]
% \caption{Juntas dos esqueletos presentes no \ac{egait}}
\label{tbl:skeleton-coord}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\rowcolor[HTML]{C0C0C0} 
\textbf{ID} & \textbf{Joint}    & \textbf{ID} & \textbf{Joint}   \\ \hline
\rowcolor[HTML]{EFEFEF} 
0           & Root              & 8           & Right Elbow \\ \hline
\rowcolor[HTML]{EFEFEF} 
1           & Spine            & 9           & Right Hand      \\ \hline
\rowcolor[HTML]{EFEFEF} 
2           & Neck           & 10          & Left Hip \\ \hline
\rowcolor[HTML]{EFEFEF} 
3           & Head            & 11          & Left Knee  \\ \hline
\rowcolor[HTML]{EFEFEF} 
4           & Left Shoulder    & 12          & Left Foot      \\ \hline
\rowcolor[HTML]{EFEFEF} 
5           & Left Elbow & 13          & Right Hip  \\ \hline
\rowcolor[HTML]{EFEFEF} 
6           & Left Hand      & 14          & Right Knee   \\ \hline
\rowcolor[HTML]{EFEFEF} 
7           & Right Shoulder     & 15          & Right Foot       \\ \hline
\end{tabular}
\end{table}

==> tables/table-steppp-params.tex <==
\begin{table}[H]
\caption{Training parameters for ST-Gait++.}
\label{tbl:steppp-params}
\centering
\begin{tabular}{lc}
\hline
\textbf{Parameter}          & \textbf{Values} \\ \hline
Train/Validation/Test Split & 7:2:1           \\
Epochs                      & 200             \\
Batch Size                  & 8               \\
Optimizer                   & RMSProp         \\
Basic Learning Rate         & 0.01            \\
Momentum                    & 0.9             \\
Weight Decay                & $3 \times 10^{-4}$               \\
GCN Initializer             & Offset          \\ \hline
\end{tabular}
\end{table}
